NovAScore: A New Automated Metric for Evaluating Document Level Novelty

The rapid expansion of online content has intensified the issue of information redundancy, underscoring the need for solutions that can identify genuinely new information. Despite this challenge, the research community has seen a decline in focus on novelty detection, particularly with the rise of large language models (LLMs). Additionally, previous approaches have relied heavily on human annotation, which is time-consuming, costly, and particularly challenging when annotators must compare a target document against a vast number of historical documents. In this work, we introduce NovAScore (Novelty Evaluation in Atomicity Score), an automated metric for evaluating document-level novelty. NovAScore aggregates the novelty and salience scores of atomic information, providing high interpretability and a detailed analysis of a document's novelty. With its dynamic weight adjustment scheme, NovAScore offers enhanced flexibility and an additional dimension to assess both the novelty level and the importance of information within a document. Our experiments show that NovAScore strongly correlates with human judgments of novelty, achieving a 0.626 Point-Biserial correlation on the TAP-DLND 1.0 dataset and a 0.920 Pearson correlation on an internal human-annotated dataset.

==> tables/novelty_corr_human.tex <==
\begin{table}[ht]
\centering
\resizebox{0.48\textwidth}{!}
{
    \begin{tabular}{ccc}
    \toprule
    \multicolumn{2}{c}{\textbf{Novelty Evaluator} $\rightarrow$} & CosSim & NLI & QA \\
    \cmidrule{3-5}
    \textbf{\textit{Task}} $\downarrow$ & \textbf{Metric} $\downarrow$ \\
    \multirow{2}{*}{\makecell[c]{\textit{Binary}\\ \textit{Classification}}} & Accuracy & 0.83 & \textbf{0.94} & 0.91 \\
    & Macro F1 & 0.71 & \textbf{0.84} & 0.80 \\
    \midrule
    % \multicolumn{4}{c}{\textit{{\nova} Correlation}} \\
    \multirow{2}{*}{\makecell[c]{{\nova}\\ \textit{Correlation}}} &
    Pearson & 0.748 & \textbf{0.920} & 0.843 \\
     & $p$-Value & 8.5e-07 & \textbf{9.6e-14} & 2.9e-09 \\
    \bottomrule
    \end{tabular}
}
\caption{Binary classification results and {\nova} correlation of each novelty evaluator. Binary classification compares each evaluator’s ACU novelty classification with human annotations. {\nova} correlation shows the correlation between {\nova}$_{\text{human}}$ and automated {\nova} using each evaluator.}
\label{tab:novelty_corr_human}
\end{table}

% \begin{table}[ht]
% \centering
% \resizebox{0.48\textwidth}{!}
% {
%     \begin{tabular}{lccc}
%     \toprule
%     \textbf{Novelty Evaluator}$\rightarrow$ & CosSim & NLI & QA \\
%     \cmidrule{2-4}
%     \multicolumn{4}{c}{\textit{Binary Classification}} \\
%     Accuracy & 0.87 & \textbf{0.97} & 0.90 \\
%     Macro F1 & 0.61 & \textbf{0.77} & 0.64 \\
%     \midrule
%     \multicolumn{4}{c}{\textit{{\nova} Correlation}} \\
%     Pearson & 0.796 & \textbf{0.914} & 0.737 \\
%     $p$-Value & 5.2e-08 & \textbf{2.8e-13} & 9.0e-05 \\
%     \bottomrule
%     \end{tabular}
% }
% \caption{}
% \label{tab:novelty_corr_human_temp}
% \end{table}

% \begin{table}[ht]
% \centering
% \resizebox{0.48\textwidth}{!}
% {
%     \begin{tabular}{lcccc}
%     \toprule
%     \textbf{Metric $\rightarrow$} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} & \textbf{Support} \\
%     \cmidrule{2-5}
%     \textbf{Class $\downarrow$} \\
%     Non-Novel & 0.45 & 0.70 & 0.55 & 44 \\
%     Novel & 0.99 & 0.97 & 0.98 & 1507 \\
%     \midrule
%     Accuracy & & & 0.97 & 1551 \\
%     Macro Avg & 0.72 & 0.84 & 0.77 & 1551 \\
%     \bottomrule
%     \end{tabular}
% }
% \caption{nli classification round 0}
% \label{tab:temp}
% \end{table}

% \begin{table}[ht]
% \centering
% \resizebox{0.48\textwidth}{!}
% {
%     \begin{tabular}{lcccc}
%     \toprule
%     \textbf{Metric $\rightarrow$} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} & \textbf{Support} \\
%     \cmidrule{2-5}
%     \textbf{Class $\downarrow$} \\
%     Non-Novel & 0.72 & 0.71 & 0.72 & 96 \\
%     Novel & 0.96 & 0.97 & 0.96 & 747 \\
%     \midrule
%     Accuracy & & & 0.94 & 843 \\
%     Macro Avg & 0.84 & 0.84 & 0.84 & 843 \\
%     \bottomrule
%     \end{tabular}
% }
% \caption{nli classification round 1}
% \label{tab:temp}
% \end{table}

% \begin{table}[ht]
% \centering
% \resizebox{0.48\textwidth}{!}
% {
%     \begin{tabular}{lcccc}
%     \toprule
%     \textbf{Metric $\rightarrow$} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} & \textbf{Support} \\
%     \cmidrule{2-5}
%     \textbf{Class $\downarrow$} \\
%     Non-Salient & 0.87 & 0.75 & 0.81 & 1277 \\
%     Salient & 0.30 & 0.50 & 0.37 & 274 \\
%     \midrule
%     Accuracy & & & 0.70 & 1551 \\
%     Macro Avg & 0.59 & 0.62 & 0.59 & 1551 \\
%     \bottomrule
%     \end{tabular}
% }
% \caption{salience round 0}
% \label{tab:temp}
% \end{table}

% \begin{table}[ht]
% \centering
% \resizebox{0.48\textwidth}{!}
% {
%     \begin{tabular}{lcccc}
%     \toprule
%     \textbf{Metric $\rightarrow$} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} & \textbf{Support} \\
%     \cmidrule{2-5}
%     \textbf{Class $\downarrow$} \\
%     Non-Salient & 0.64 & 0.56 & 0.59 & 531 \\
%     Salient & 0.38 & 0.46 & 0.42 & 312 \\
%     \midrule
%     Accuracy & & & 0.52 & 843 \\
%     Macro Avg & 0.51 & 0.51 & 0.51 & 843 \\
%     \bottomrule
%     \end{tabular}
% }
% \caption{salience round 1}
% \label{tab:temp}
% \end{table}

% \begin{table}[ht]
% \centering
% \resizebox{0.48\textwidth}{!}
% {
%     \begin{tabular}{lcc}
%     \toprule
%     \textbf{Annotation Round $\rightarrow$} & \textbf{Round 0} & \textbf{Round 1} \\
%     \cmidrule{2-3}
%     \multicolumn{3}{c}{\textit{Expected Novel ACUs}} \\
%     Accuracy & 1.0 & 0.99 \\
%     Weighted F1 & 1.0 & 1.0 \\
%     \midrule
%     \multicolumn{3}{c}{\textit{Expected Non-Novel ACUs}} \\
%     Accuracy & 0.63 & 0.82 \\
%     Weighted F1 & 0.77 & 0.90 \\
%     \midrule
%     \multicolumn{3}{c}{\textit{GPT-Extracted ACUs Quality}} \\
%     Incorrect Rate & 0.3\% & 0.0\% \\
%     Redundant Rate & 2.1\% & 0.1\% \\
%     \bottomrule
%     \end{tabular}
% }
% \caption{s}
% \label{tab:temp}
% \end{table}


